ECon: On the Detection and Resolution of Evidence Conflicts

The rise of large language models (LLMs) has significantly influenced the quality of information in decision-making systems, leading to the prevalence of AI-generated content and challenges in detecting misinformation and managing conflicting information, or "inter-evidence conflicts." This study introduces a method for generating diverse, validated evidence conflicts to simulate real-world misinformation scenarios. We evaluate conflict detection methods, including Natural Language Inference (NLI) models, factual consistency (FC) models, and LLMs, on these conflicts (RQ1) and analyze LLMs' conflict resolution behaviors (RQ2). Our key findings include: (1) NLI and LLM models exhibit high precision in detecting answer conflicts, though weaker models suffer from low recall; (2) FC models struggle with lexically similar answer conflicts, while NLI and LLM models handle these better; and (3) stronger models like GPT-4 show robust performance, especially with nuanced conflicts. For conflict resolution, LLMs often favor one piece of conflicting evidence without justification and rely on internal knowledge if they have prior beliefs.

==> floats/in-line-intensity-accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
  \resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c|}{}                                 & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{Conflict Intensity}}} \\ \cline{2-5} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Model}}} & 1                     & 2                     & 3                      & 4                     \\ \hline
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\textit{Large language models}}                                                                             \\
\multicolumn{1}{l|}{Mixtral 8x7B}                     & 7.0                   & 23.3                  & 35.3                   & 49.0                  \\
\multicolumn{1}{l|}{Llama-3 8B Inst.}                 & 54.8                  & 85.6                  & 93.1                   & 99.0                  \\
\multicolumn{1}{l|}{Llama-3 70B Inst.}                & 68.9                  & 92.5                  & 99.0                   & 100.0                 \\
\multicolumn{1}{l|}{Claude 3.0 Haiku}                 & 38.6                  & 70.6                  & 83.3                   & 93.9                  \\
\multicolumn{1}{l|}{Claude 3.0 Sonnet}                & 73.3                  & 96.6                  & 99.0                   & 100.0                 \\
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\textit{Factual consistency}}                                                                               \\
\multicolumn{1}{l|}{AlignScore-base}                  & 23.3                  & 54.1                  & 80.4                   & 96.9                  \\
\multicolumn{1}{l|}{AlignScore-large}                 & 27.6                  & 69.9                  & 90.2                   & 99.0                  \\
\multicolumn{1}{l|}{MiniCheck-R}                      & 48.3                  & 63.7                  & 71.6                   & 88.8                  \\
\multicolumn{1}{l|}{MiniCheck-D}                      & 89.0                  & 94.5                  & 96.1                   & 92.9                  \\
\multicolumn{1}{l|}{MiniCheck-FT5}                    & 65.8                  & 80.8                  & 86.3                   & 94.9                  \\
\multicolumn{5}{l}{\cellcolor[HTML]{EFEFEF}\textit{NLI models}}                                                                                        \\
\multicolumn{1}{l|}{NLI-xlarge (Max)}                 & 21.1                  & 48.0                  & 65.7                   & 88.8                  \\
\multicolumn{1}{l|}{NLI-xlarge (C\textgreater{}E)}    & 21.9                  & 48.0                  & 66.7                   & 88.8                  \\
\multicolumn{1}{l|}{NLI-xxlarge (Max)}                & 54.4                  & 87.0                  & 97.1                   & 100.0                 \\
\multicolumn{1}{l|}{NLI-xxlarge (C\textgreater{}E)}   & 71.9                  & 94.5                  & 100.0                  & 100.0                 \\ \bottomrule
\end{tabular}
}
\caption{Detection recall (\%) on varying intensity of factoid conflicts.}
\end{table}

==> floats/in-line-overlap-accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\small
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{c|}{}                                 & \multicolumn{3}{c}{\textbf{Overlap}}                                           \\ \cline{2-4} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Model}}} & 1                        & 2                        & 3                        \\ \hline
\multicolumn{4}{l}{\cellcolor[HTML]{EFEFEF}\textit{Large language models}}                                                             \\
\multicolumn{1}{l|}{Mixtral 8x7B}                     & 17.8                     & 17.8                     & 15.9                     \\
\multicolumn{1}{l|}{Llama-3 8B Inst.}                 & 62.7                     & 70.7                     & 69.2                     \\
\multicolumn{1}{l|}{Llama-3 70B Inst.}                & 72.9                     & 75.9                     & 68.8                     \\
\multicolumn{1}{l|}{Claude 3.0 Haiku}                 & 54.2                     & 51.2                     & 55.8                     \\
\multicolumn{1}{l|}{Claude 3.0 Sonnet}                & 81.4                     & 77.0                     & 72.6                     \\
\multicolumn{4}{l}{\cellcolor[HTML]{EFEFEF}\textit{Factual consistency}}                                                               \\
\multicolumn{1}{l|}{AlignScore-base}                  & 81.4                     & 50.0                     & 20.7                     \\
\multicolumn{1}{l|}{AlignScore-large}                 & 90.7                     & 61.5                     & 35.1                     \\
\multicolumn{1}{l|}{MiniCheck-R}                      & \multicolumn{1}{l}{64.4} & \multicolumn{1}{l}{65.5} & \multicolumn{1}{l}{69.2} \\
\multicolumn{1}{l|}{MiniCheck-D}                      & \multicolumn{1}{l}{93.2} & \multicolumn{1}{l}{94.3} & \multicolumn{1}{l}{94.7} \\
\multicolumn{1}{l|}{MiniCheck-FT5}                    & \multicolumn{1}{l}{83.1} & \multicolumn{1}{l}{80.5} & \multicolumn{1}{l}{78.9} \\
\multicolumn{4}{l}{\cellcolor[HTML]{EFEFEF}\textit{NLI models}}                                                                        \\
\multicolumn{1}{l|}{NLI-xlarge (Max)}                 & \multicolumn{1}{l}{45.8} & \multicolumn{1}{l}{46.3} & \multicolumn{1}{l}{49.3} \\
\multicolumn{1}{l|}{NLI-xlarge (C\textgreater{}E)}    & \multicolumn{1}{l}{45.8} & \multicolumn{1}{l}{46.3} & \multicolumn{1}{l}{49.3} \\
\multicolumn{1}{l|}{NLI-xxlarge (Max)}                & \multicolumn{1}{l}{60.6} & \multicolumn{1}{l}{70.7} & \multicolumn{1}{l}{66.4} \\
\multicolumn{1}{l|}{NLI-xxlarge (C\textgreater{}E)}   & \multicolumn{1}{l}{60.6} & \multicolumn{1}{l}{70.7} & \multicolumn{1}{l}{66.4} \\ \bottomrule
\end{tabular}
\caption{Detection recall (\%) on varying intensity of corroborating factoids.}
\label{tab:intensity-corroboration}
\end{table}

==> sections/answer_conflicts.tex <==

\section{Answer conflicts detection}
\label{sec:answer-conflict}


A common type of evidence conflict source from where models suggest conflicting answers to a question, i.e., answer conflicts.
In this section, we develop a pipeline to generate and validate evidence pairs that have answer conflicts.
We analyze models' conflict detection ability on the generated set.
In addition, we test models on hard answer-conflict created by answer-centric pollution to simulate potential malicious attacks on the Internet. 

\subsection{Evaluation setup}
We base our evaluation on two public datasets, NaturalQuestions (NQ; \citealp{lee2019latent}) and ComplexWebQuestions (CWQ; \citealp{talmor2018web}). 
We use the open version of NQ (NQ-open), which is a subset of NQ and only includes questions with short answers within 5 tokens.
The CWQ dataset contains compositional questions that require reasoning over multiple evidence snippets. 
Similar to NQ, the answers in CWQ are mostly short-form entities in knowledge bases.

For each question and its answer ($q$, $a_0$; e.g.,  \textit{$q$=``who wrote the music for somewhere in time? '', $a_0$=``John Barry''}), we generate a set of alternative answers $\{a_1, a_2, \cdots\}$.
% \noindent \textbf{Alternative answer generation} 
% First, a set of alternative answers $\{a_1, a_2, \cdots\}$ are generated given $q$ and $a_0$.
$$\{a_i|i=[1, 2, \cdots]\} = \texttt{AnswerGen}(q, a_0) $$

% Then, for each alternative answer, we generate a corresponding supporting evidence set $\{e_1, e_2, \cdots\}$.
% \noindent \textbf{Supporting evidence generation}
Then, a piece of supporting evidence $e_i$ is generated for each $a_i (i\in\{0, 1, 2, \cdots\})$.
$$e_i = \texttt{EvidenceGen}(q, a_i) $$

Here, we adopt \texttt{llama3-70b-instruct} to generate answers and evidence.
When generating the evidence, we control the length of each piece of text with instructions.
Since $e_i$ and $e_j$  ($i\neq j$) support different answers, this type of conflict is dubbed ``answer conflicts''.

% \noindent \textbf{Pair construction} 
The conflicting pairs are then constructed by selecting ($e_i$, $e_j$; $i\neq j$) such that they support conflicting answers ($a_i$, $a_j$) to a same question $q$. 
On the other hand, non-conflicting pairs are picked from evidence suggesting the same answer ($e_{i(1)}$, $e_{i(2)}$, ...).

\noindent \textbf{Quality check}
To generate evidence at scale, automatic checking of generation quality is crucial \cite{xie2023adaptive}. 
All the evidence is checked by a two-step program to make sure they can be used to derive the intended answers: 
% This check consists of two steps.
(1) an NLI check (such that $q$ and $e_i$ entails $a_i$).
% \tianhang{what dose $e_{i\rightarrow j}$ mean?}
(2) an LLM reasoning check (such that an LLM can infer $a_i$ when given $q$ and $e_i$).
A piece of evidence is filtered out when it fails on any of the steps.


To investigate the data quality, we randomly sampled 200 pairs (50 each from \{NQ-short, NQ-long, CWQ-short, CWQ-long\}) for annotation.
Given a question $q$, each pair or evidence ($e_i, e_j$) is annotated by three independent annotators to determine its label from \{\texttt{Conflicting},\space \texttt{Non-conflicting},\space \texttt{Not sure}\}.
The Fleiss' $\kappa$~\cite{fleiss1971measuring} among the annotators is 71.2\%, which indicates substantial inter-annotator agreement.
Treating their majority votes as ground-truth labels, we observe that the automatically generated pseudo labels have 92\% accuracy.
We observe that question ambiguity is the major reason for wrong generations, which admits multiple valid answers depending on disambiguation \cite{min2020ambigqa, zhang2021situatedqa}. For example, for ``who was the president of the United States?'', there are many possible correct answers depending on the exact date.

% \noindent \textbf{Data analysis} 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/type_ratio.pdf}
    \caption{Type distributions of the answer and factoid conflicts.}
    \label{fig:type_dist}
\end{figure}

% \noindent \textit{Types of conflicts.}
To investigate the data composition, we manually annotate types of conflicts for the sampled pairs.
The ratio of conflict types is presented in Figure~\ref{fig:type_dist}.
Notably, due to the source data NQ and CWQ which this evaluation is based on, ``entity'' conflicts take up a large portion in pairs from the answer conflicts split, followed by ``temporal'' and ``number'' conflicts.
Example pairs can be found in Table~\ref{tab:main_examples}.
% This is probably because are generated from NQ.

% \noindent \textit{Generation errors.}

% 2. Additionally, we observe cases where the actual answer strings differ but convey similar meanings, such as "Summer 1979" versus "July 1979". 
% 3. Another intriguing type of generation error we identify is the "right for the wrong reason" scenario. In some answer conflict cases, the evidence passages contain conflicting information outside of the answer span itself. 
% 4. Similarly, we also observe the "wrong for the right reason" scenario, in which two evidence passages imply different answers for the question, yet their explanatory text is similar.



\subsection{Answer conflict detection}
\label{sec:identify-answer-conflict}
% \tianhang{Analysis for answer conflict detection?}

\input{floats/answer-conflict-label1-length}
% Setting
We test conflict detection models ($\S$~\ref{sec:task-definition}) on the evidence pairs.
The results are presented in Table~\ref{tab:answer-conflict-length}. 
We have several observations:

% Overall trends
\noindent \textbf{NLI and LLM models are high precision conflict detectors.}
As a general trend, the NLI and LLM models have high precision but low recall on the detection task. 
Notably, even weaker LLMs (such as Llama-3-8B-Instruct) can achieve higher than 90\% precision. 
Since the performance gap is mainly on the low recall, it is clear that NLI and LLM detectors are relatively conservative about their conflict predictions.
However, this trend is observed on factual consistency models.

% Impact of context length on NLI models
\noindent \textbf{NLI detectors are sensitive to context lengths.}
Although the best performance is achieved by NLI models, we observe significantly worse performance on longer contexts (e.g., -18.2\% F1 for NLI-xlarge (C>E)) for some NLI detectors.
One possible reason is that they are trained on sentence-level datasets, and hence could suffer from the generalization here.
In contrast, most LMs and factual consistency models are relatively robust to context length. 


% We further analyze models' predictions.
% \noindent \textbf{Analysis on model answers (and case study)}
% We sample errors from each group of models.
% Analysis and statistics of the errors are presented.
% \thought{
% (Since the recall on class 1 is low, questions that worth further investigation: 
% "what kind of conflicts are ignored most frequently?")
% }






\subsection{Conflict detection under pollution attacks}
% \tianhang{I think we can clarify the difference between this task and answer conflict and make it more coherent with the text above}
\input{floats/pollution_example}

\input{floats/pollution_breakdown_acc}

% In the era of LLMs, the Internet could be flooded with machine generated contents with misinformation. 
% On the one hand, hallucination remains one of the unsolved issues, where models could produce ``seemingly true'' evidence to pollute the web \cite{ji2023survey}.
% On the other hand, malicious attacks are much easier than before, where misinformation can be manufactured through automatic generation and spread to the end-point users \cite{pan2023risk}.

In addition to the vanilla setting, we investigate a setting that is supposed to be harder: we evaluate whether conflict detectors will be affected by the machine-generated misinformation, sourced from malicious modifications over existing evidence.
We adopt the \textsc{Revise} misinformation pollution attack~\cite{pan2023risk} to inject conflicting facts by modifying existing evidence.
Here, evidence (e.g., $e_i$ that supports answer $a_i$) is polluted to support another answer (e.g., $a_j$) while making minimum necessary modifications (e.g., $e_{i\rightarrow j}$ supports $a_j$).
$$e_{i\rightarrow j} = \texttt{Modify}(q, a_i, a_j, e_i) $$
Note that $e_{i\rightarrow j}$ includes much of the same details as in $e_i$ despite supporting another answer $a_j$.
A pollution example is shown in Table~\ref{tab:pollution-attack}.
We consider the following three types of conflicting pairs:
% We then observe the detection for pairs ($e_{i\rightarrow j}$, $e_i$), ($e_{i\rightarrow j}$, $e_j$), and so on.
\begin{itemize}[leftmargin=*]
    \item ($e_A$, $e_B$): Direct conflict. The two pieces of evidence are different and independently support the respective answer.
    \item ($e_{A\rightarrow B}^1$, $e_A^1$): Close polluted conflict. $e_{A\rightarrow B}^1$ is modified from $e_A^1$, and hence they have close details but suggest different answers.
    \item ($e_{A\rightarrow B}^1$, $e_A^2$): Far polluted conflict. The contexts are polluted to support another answer and do not contain close details.
    % \item \tianhang{I think it is also a direct conflict?}
\end{itemize}

\noindent \textbf{NLI and LLM models are good at detecting ``close polluted conflicts'' in pollution attacks.}
Model detection results are reported in Table~\ref{tab:breakdown_answer_acc}.
% General observations
Notably, LLM and NLI models tend to detect the close polluted conflicts the best, while having similar performance on direct conflicts and far-polluted conflicts. 
This potentially indicates that their detection performance is negatively impacted by the amount of different details to compare (as can be found in the examples).

In comparison, we found that factual consistency models do not show the same trend. 
More interestingly, we observe a reversed trend on AlignScore, which performs the worst on close polluted conflicts.
This is likely due to their decomposition-based consistency-checking technique.
Since the overall factual consistency is high except for the answer-related details, detecting close polluted conflicts is like finding a needle in a haystack for these models.

% \noindent \textbf{``Far polluted conflicts''}

% extended discussion on factual consistency and ...

% Breakdown on types of pairs

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/label_1_diff_shortlist.png}
%     \caption{Model performance change (\%). }
%     \label{fig:enter-label}
% \end{figure}






==> sections/factoid_conflicts.tex <==
\section{Factoid conflicts detection}
\label{sec:factoid-conflict}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/factoid-conflict.png}
    \caption{Evidence pair generation with factoid conflicts.}
    \label{fig:factoid-conflicts}
\end{figure}

% \thought{Intro to factoid conflicts}
Though answer conflicts are a good starting point to estimate and test models' conflict detection abilities, they are less general.
For instance, upon deeper analysis (Figure~\ref{fig:type_dist}), we found that answer conflicts are predominantly about contradictory entities, dates, or numbers.
However, real-world evidence conflicts include other types such as semantic perturbation \cite{jia2017adversarial, chen2022rich}, and might have varying intensity or degrees.
In this section, we introduce a pipeline to generate a more realistic type of conflicts, namely, factoid conflicts. 


\subsection{Evaluation setup}
In this evaluation, we assume each piece of evidence $e^i$ can be expressed by a set of factoids $S^i=\{s_1^i, s_2^i, \cdots\}$.
Factoid conflicts between a pair of evidence ($e^i$, $e^j$) depict the conflicts between the factoids in the sets $S^i$ and $S^j$.
We base the evaluation on StrategyQA~\cite{geva2021strategyqa}, where questions are backed with human-verified factoids for reaching conclusions.
As shown in Figure~\ref{fig:factoid-conflicts}, given a question $q$, we perturb the factoids in $S$ to obtain conflicting factoids ($s_k \rightarrow s_k^p$; $s_k^p$ is a factoid in the perturbed set $S^p$).
The factoids are semantically perturbed using a perturbation $p$ to create conflicting factoids\footnote{Previous work have explored entity substitution \cite{longpre2021entity} and semantic perturbation \cite{chen2022rich}.
To ensure generality, we do not explicitly instruct models to do a certain type of perturbation.}.
$$s_k^p = \texttt{Perturb}(s_k) $$
Then, an evidence is generated based on a set of factoids selected from $S$ or $S^p$.
% \noindent \textbf{Factoids to evidence generation}
% Based on the question, the original and perturbed factoids, an evidence is generated:
$$e^i = \texttt{EvidenceGen}(q, \{s_1^{p_1^i}, s_2^{p_2^i}, \cdots\}) $$
where $p_k^i \in \{0, 1\}$ indicates whether the $k$-th factoid is perturbed. 
Then, $p^i=[p_1^i, p_2^i, \cdots]$ is the perturbation indicator vector.


\noindent \textbf{Quality check}
Each piece of generated evidence $e^i$ is checked by an NLI model to guarantee that 
(1) it entails all the factoids used to generate itself, i.e., $\forall k, e^i$ entails $s_k^{p_k^i}$; and
(2) it contradicts all the factoids not used, i.e., $\forall k, e^i$ contradicts $s_k^{(1-p_k^i)}$.
With this quality check, the intensity of conflicts between a pair of evidence $e^i$ and $e^j$ can be approximated by the following ratio ($\oplus$ is the exclusive or operation):
$$\hat f(e^i, e^j) = \frac{\text{Sum}(p^i \oplus p^j)}{n}$$

\subsection{Analysis on data}
% To investigate the quality of the generated data, we ask three domain-experts to annotate on the evidence pairs from both answer- and factoid-conflict splits.
To evaluate how the approximation $\hat f(e^i, e^j)$ is linked to the actual perceived level of conflicts, two annotators are asked to select their subjective feeling over the degree of conflicts from \{ \texttt{Non-conflicting}, \texttt{Weakly conflicting},  \texttt{Conflicting}, \texttt{Strongly conflicting}\}. 
The labels are converted to continuous values within [0, 1].
The Pearson correlation coefficient $\rho$ is 0.622 with p-value $1.4\times 10^{-6}$, which suggests significant positive correlation between the pseudo labels and human's subjective perception over the intensity of conflicts.
Details of the annotation process are in Appendix~\ref{sec:appendix-annotation}.



% \noindent \textbf{Data analysis}
% \noindent \textit{Types of conflicts}
The ratio of conflict types is presented in Figure~\ref{fig:type_dist} and examples in Table~\ref{tab:main_examples}.
Unlike the answer conflicts split, types of factoid conflicts split shows higher diversity, where ``Negation'' and ``Degree'' take up a considerable portion of data, which are sourced from the perturbation over factoids.
% Unlike answer conflicts, factoid conflicts do not necessarily indicate conflicting answers. 

% \noindent \textit{Generation errors}
% % ``Right for the wrong reason''. 
% In factoid conflicts, evidence suggest the same label ``yes/no'' with different or contradicting facts.


\subsection{Detection results}
\label{sec:intensity-of-conflicts}
\input{floats/inline-intensity-acc}

With the factoid conflict generation pipeline, we are able to generate evidence pairs with varying intensities of conflicts and corroboration.
\begin{itemize}[leftmargin=*]
    \item Intensity of conflict. We create evidence pairs with varying level of conflict $\hat f(e^i, e^j)$ by controlling the number of different factoids selected from $S$ and $S^p$. The total factoid number in each evidence is fixed to 4, and the evidence length is controlled by instruction.
    \item Intensity of corroboration. To evaluate the effect of corroborating factoids\footnote{Corroborating factoids refer to those used in generating both evidence. For instance, $s_0$ in Figure~\ref{fig:factoid-conflicts}. } in detection, we control the level of corroboration by selecting (1) one pair of conflicting factoids and (2) varying number of corroborating factoids.
\end{itemize}
% \tianhang{I think the two itemize are not factoid conflicts detection results, could it be merged into the setup section?}

Results are presented in Table~\ref{tab:intensity-results}. 
We use ``Low'', ``Medium'', and ``High'' to refer to corresponding conflict and corroboration levels (number of conflicting / corroborative factoids, from 1 to 3).

\noindent \textbf{Models tend to detect conflicts with higher intensity, but stronger models are more robust on nuanced conflicts.}
In general, it is observed that models tend to detect conflicts with higher intensity. 
While trend is universal to all models, stronger models such as Llama-3 70B, Claude 3 Sonnet, GPT-4, MiniCheck-D, and NLI-xxlarge are much more robust than weaker models.
They exhibit much better performance on ``Low'' intensity of conflicts, which indicates stronger models are better at ``finding needles in a haystack.''



\noindent \textbf{Corroborating factoids do not matter very much for most models.}
In comparison, most models are relatively robust as the level of corroboration increases.
As the only exception, AlignScore is significantly influenced by the intensity of conflicts in both cases, which is possibly because of its sentence-wise score computation mechanism.
% \tianhang{could explain more?}


% \input{floats/in-line-intensity-accuracy}

% \input{floats/in-line-overlap-accuracy}


% \noindent \textbf{Pair construction}

% \noindent \textbf{Results}


% (1) Whether the order of factoids used to generate evidence affect models' performance in identifying conflicts?

% (2) How does the intensity of conflict affect models' performance? Pairs of evidence with more conflict information are considered to have a higher level of conflict intensity.


% \subsection{Factoid conflicts: intensity of corroborations}
% \label{sec:identify-corroboration}


% \noindent \textbf{Pair construction}

% \noindent \textbf{Results}

% Results are shown in table~\ref{tab:intensity-corroboration}.


==> sections/misc.tex <==
\section{Miscellaneous}
\label{sec:misc}

We present miscellaneous developmental results in this section.
It is temporary and would be removed in the submission.

\subsection{Ambiguity, situated questions, and evidence conflict}
\noindent \textbf{Ambiguity in open-domain QA.} 
\citet{min2020ambigqa} proposed AmbigQA based on the open-domain QA questions, where it annotated ambiguous questions that could result in multiple answers (e.g. when did the Harry Potter movie came out?).
Based on different disambiguations, these questions have different answers that are all valid.

SituatedQA: \citet{zhang2021situatedqa} explores how extra-linguistic contexts can affect open-domain QA. 
Their study reveals that current systems fail to adapt to shifts in the \underline{temporal or geographical} context. For example: ``which COVID-19 vaccines have been authorized for adults in the US?'' has time-dependent answers.

ASQA: 

\noindent \textbf{Relationship with evidence conflict.}
Ambiguity / context-dependent questions might serves as a source of evidence conflict. 
For instance, in the above example from \cite{zhang2021situatedqa}, the retrieved evidence might contradicts each other as both up-to-date and outdated evidence might occur in the result.
(Dec 18, 2014 -> Moderna, Pfizer; Apr 10, 2021 -> Moderna, Pfizer, J\&J)


\subsection{Relationship between ``Agreement score'' and ``Conflict score''?}
They are different measurements. 
For instance, pieces of evidence with low agreement might indicate that they talk about different things, but they are not necessarily very conflicting. 

(This one is minor and probably should not be mentioned.)
High agreement evidence do not have to have low conflict level, as they might be \textit{conditioned} on different aspects.

On the other hand, conflicting evidence must have low agreement? (This one needs experimental results.)

\subsection{Can LLMs detect knowledge conflicts?}

Our qualitative results have shown that LLMs can indeed detect potential conflicts in retrieval results.


\subsection{Can \methodname be used to detect confirmation bias?}


The confirmation bias models the phenomenon that, when faced with conflicting evidence, LLMs tend to highlight the evidence that confirms its prior beliefs \cite{xie2023adaptive}.


\subsection{Any theoretical guidance on how to model the degree of evidence conflicts?}

For belief-evidence conflict, previous works rely on memorization ratio to reflect the degree (in a controlled data setting).

Search for \textit{triangulation} in social science, \textit{evidence theory} in mathematics.

\subsection{Psychology related}
\begin{itemize}
    \item \textit{Motivated reasoning.} Through the mechanism of motivated reasoning, people tend to seek out, pay attention to, remember, and trust information which corroborates their prior attitudes and discredits opposing information. (relevant citations can be found at \cite{filkukova2021should})
    \item \textit{Confirmation bias.} Confirmation bias is the tendency to search for, interpret, favor, and recall information in a way that confirms or supports one's prior beliefs or values.[1] People display this bias when they select information that supports their views, ignoring contrary information, or when they interpret ambiguous evidence as supporting their existing attitudes. (Wikipedia)
    \item \textit{Cognitive dissonance.} Individuals are compelled to initiate motivated reasoning to lessen the amount of cognitive dissonance they feel. Cognitive dissonance is the feeling of psychological and physiological stress and uneasiness between two conflicting cognitive and/or emotional elements (such as the desire to smoke, knowing it is unhealthy). (Wikipedia)
    \item Motivated reasoning, confirmation bias and cognitive dissonance are closely related to each other. 


\end{itemize}


\subsection{Other interesting facts/concepts}
\begin{itemize}
    \item The amount of misinformation on Internet platforms is on the rise. (Lazer et al., 2018)
    \item A recent study found that on social media (Twitter) false news spread even faster than true news (Vosoughi et al.,2018).

    \item \textit{Triangulation (social science)} is a research strategy that involves using multiple datasets, methods, theories, and/or investigators to address a research question. It can help you to validate and enrich your findings, as well as avoid research biases. Our method is closely related to data triangulation.
    \item \textit{Credible sources.} (Primary, Secondary, Tertiary).

\end{itemize}




\subsection{(Deprecated) Data construction}
There are two dimensions to consider to construct a conflicting evidence benchmark for later evaluation use, i.e. the source of data and the construction methods.

\noindent \textbf{Source data}
According to the type of answers, we can split the existing data source into two groups. 
\begin{itemize}
    \item \textit{Simple questions with clear and short answers.} 
    NQ-open \cite{lee2019latent} is an open version of the NaturalQuestions dataset, where questions with short answers (discard answers with more than 5 tokens, who, when, where, etc.) and kept. The given evidence document is discarded. 

    MythQA \cite{bai2023mythqa} contains entity questions and yes/no questions on the controversial topics (listed on wikipedia) in the ``Science, biology, and health'' and ``politics and economics'' sections\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:List_of_controversial_issues}}. 
    It has similar answer format as NQ-open (short answers with less than 5 tokens).
    Each entity question has 3.5 distinct answers on average (for yes/no questions, there are 2).

    AmbigNQ \cite{min2020ambigqa} is constructed based on NQ-open, where it annotated ambiguous questions from NQ-open. Also, SituatedQA \cite{zhang2021situatedqa} provides temporal and geological disambiguation for questions.
    
    Other candidates: Similar datasets include TriviaQA, Web-questions, etc., which we could explore in the future. 
    Yes/No answers: StrategyQA, BoolQ. 
    
    \item \textit{Complex questions with (controversial) long-form answers.}
    This includes the compexity brought by the questions (e.g., a controversial topic, or question that requires multi-hop reasoning) or by the form of answers (e.g., long-form answers).

    Long-form QA:
    ELI5 \cite{eli5_lfqa} explain like i am 5 collected from reddit.
    ASQA \cite{stelmakh2022asqa} extend from ...

    Controversial topics: 
    CovidNews.
    climate change (Climate-Fever), flat-earth.
    
   Requiring CoT reasoning:  StrategyQA. 

    
Multi-hop fact verification data, such as 2WikiMultiHopQA,  HotpotQA (comparison), 
\end{itemize}


\noindent \textbf{Conflicting data construction}
To prepare data with conflicting evidence and evidence-beliefs, we consider two data construction methods.
\begin{itemize}
    \item \textit{Pollution.} We conduct evidence pollution or generate counter-evidence with existing LLMs, such as ChatGPT, LLaMa. 
    This strategy has been adopted by \cite{longpre2021entity, neeman2023disentqa, xie2023adaptive, chen2022rich, pan2023risk}.

    According to the target of pollution, the method can be categorized into two kinds:
    \begin{enumerate}
        \item Answer-oriented pollution. The aim of this pollution is to alter as least details as possible such that the supporting answer changed. 

        \underline{Ground-truth: Y/N.} Whether there is conflict or not. 
        
        Automatic construction is possible.
        \item Direct pollution. This kind of pollution directly operates on evidence, without focusing on the answer.

        \underline{Ground-truth: Degree of conflicts.}
        
        Automatic construction / human annotation.
    \end{enumerate}
    We elicit possible answers and correponding supporting evidence from LLMs, and then check their quality with entailment check and consistency check, similar to \cite{xie2023adaptive}.
    The results are presented in \ref{sec:prelim-exp}
    
    {\color{blue} Try ChatGPT and LLaMa2. Consider different pollution ways, e.g. using different entity/answer to generate, or use negation, ... to generate. Try analyzing the effect of ground-truth evidence.}
    
    \item \textit{Active web search.} To reflect more realistic evidence on the internet, we also consider creating conflicting evidence sets by actively searching online.
    The conflicting evidence collected this way should be more realistic than the previous ones, and thus serves as a good test set.
    
    \underline{Ground-truth: Degree of conflicts.}

    Human annotation only.
    
    {\color{blue} How to ``actively search'' so that the evidence are conflicting? Or we can simply choose the controversial topics so that there are much conflicting evidence, e.g. CovidNews, Politifacts.}
    
    \item \textit{Others} We can use SituatedQA, AmbigQA to search for query. Or, BoolQ, wrong prediction, then search for the reason of the wrong prediction online.
    
\end{itemize}




\subsection{Typical scenarios where inter-evidence conflicts may appear (adapted from \cite{chen2022rich})}


 
\begin{enumerate}
    \item \textit{misinformation pollution} passages are adversarially edited to false information; \cite{pan2023risk}
    \item \textit{controversial topics} passages authored by people having different opinions; MythQA \cite{bai2023mythqa}
    \item \textit{ambiguity (context-dependency)} different, valid interpretations of the question; different extra-linguistic contexts. AmbigNQ \cite{min2020ambigqa} (event references, properties, entity references, answer types, time-dependency, multiple-subquestions), SituatedQA \cite{zhang2021situatedqa} (time-dependency, geo-dependency).
\end{enumerate}


\subsection{Potential source datasets}
\begin{itemize}
    \item \textit{Simple questions with short answers.} 
    NQ-open \cite{lee2019latent} is an open version of the NaturalQuestions dataset, where questions with short answers (discard answers with more than 5 tokens, who, when, where, etc.) and kept. The given evidence document is discarded. 

    MythQA \cite{bai2023mythqa} contains entity questions and yes/no questions on the controversial topics (listed on Wikipedia) in the ``Science, biology, and health'' and ``politics and economics'' sections\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:List_of_controversial_issues}}. 
    It has similar answer format as NQ-open (short answers with less than 5 tokens).
    Each entity question has 3.5 distinct answers on average (for yes/no questions, there are 2).

    AmbigNQ \cite{min2020ambigqa} is constructed based on NQ-open, where it annotated ambiguous questions from NQ-open. Also, SituatedQA \cite{zhang2021situatedqa} provides temporal and geological disambiguation for questions.
    
    Yes/No answers: StrategyQA, BoolQ. 

    
    Controversial topics: 
    CovidNews.
    climate change (Climate-Fever), flat-earth.
    Multi-hop fact verification data, such as 2WikiMultiHopQA,  HotpotQA (comparison
    
    \item \textit{Complex questions  (controversial).}

    
    
Multi-hop fact verification data, such as 2WikiMultiHopQA,  HotpotQA (comparison), 
\end{itemize}





\section{Extended discussion}
\subsection{Type of evidence conflicts}
We investigate two major types of evidence conflicts. 
\begin{enumerate}
    \item \textit{Factual conflicts.} Factual conflicts involve differences in information. 
For instance, the contradiction or consistency of factoids (or relations of factoids) contained in two pieces of evidence.
    \item \textit{Interpretation conflicts.} Interpretation conflicts, in contrast, involve varied understandings of content.  
This type of conflicts happen when two pieces of evidence use language that is open to multiple interpretations (e.g., coreference, situated on conditions like time and place, etc.)
Another typical case is when two texts present different perspectives or worldviews that are in conflict with each other  (e.g. on controversial topics such as political debate.)
\end{enumerate}


\noindent  \textit{Factual}\textbf{ }datasets include:

  \noindent  \textbf{NQ-open} \cite{lee2019latent} is an open version of the NaturalQuestions dataset, where questions with short answers (discard answers with more than 5 tokens, who, when, where, etc.) and kept. The given evidence document is discarded. 

 \noindent   \textbf{StrategyQA} \cite{geva2021strategyqa} ...
HotpotQA (comparison),

\noindent \textit{Interpretation} datasets include:

\noindent   \textbf{MythQA }\cite{bai2023mythqa} contains entity questions and yes/no questions on the controversial topics (listed on Wikipedia) in the ``Science, biology, and health'' and ``politics and economics'' sections\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:List_of_controversial_issues}}.  (has similar answer format as NQ-open)

 \noindent   \textbf{AmbigNQ} \cite{min2020ambigqa} is constructed based on NQ-open, where it annotated ambiguous questions from NQ-open. Also, SituatedQA \cite{zhang2021situatedqa} provides temporal and geological disambiguation for questions.

For the second type of conflicts, refer to section \ref{sec:misc} -1.
\placeholder {Some examples of two types of conflicts, maybe in a table}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{6311706072764_.pic.jpg}
    \caption{Procedures in generating evidence conflicts test set.}
    \label{fig:enter-label}
\end{figure}

\noindent \textbf{Fact modification and data generation with this regard}
    \begin{enumerate}
        \item \textit{Answer-oriented modification.} (for testing both \textit{factual and interpretation} conflicts) For questions with simple answers (e.g., NQ-open, MythQA, and AmbigNQ where answers are date, position, and entities), we adopt a similar strategy as in \cite{pan2023risk} by prompting LLMs to alter as least details as possible such that the supporting answer changed.  
\placeholder{ prompts and details?}

        \item \textit{Factoid-oriented modification.} (for testing \textit{intensity} of conflicts)  For more complex questions that require multi-hop reasoning or have long form answers (e.g., StrategyQA, HotpotQA, and ASQA), we develop a two-stage generation method by first modifying the \textit{factoids} in the evidence, and then select the factoids from either the original set or the modified set to create \textit{different degrees of conflicting evidence}. 
\placeholder{ details of this modification strategy: [OOOO] [OMMO], degrees etc.}  
 

    \end{enumerate} 
    
